Let the Great World Spin: Revealing the Stormy, Turbulent Nature of Young Giant Exoplanet Analogs with the Spitzer Space Telescope

We present a survey for photometric variability in young, low-mass brown dwarfs with the Spitzer Space Telescope. The 23 objects in our sample show robust signatures of youth and share properties with directly-imaged exoplanets. We present three new young objects: 2MASS J03492367$+$0635078, 2MASS J09512690 $-$8023553 and 2MASS J07180871$-$6415310. We detect variability in 13 young objects, and find that young brown dwarfs are highly likely to display variability across the L2--T4 spectral type range. In contrast, the field dwarf variability occurrence rate drops for spectral types $>$L9. We examine the variability amplitudes of young objects and find an enhancement in maximum amplitudes compared to field dwarfs. We speculate that the observed range of amplitudes within a spectral type may be influenced by secondary effects such as viewing inclination and/or rotation period. We combine our new rotation periods with the literature to investigate the effects of mass on angular momentum evolution. While high mass brown dwarfs ($>30 M_{\mathrm{Jup}}$) spin up over time, the same trend is not apparent for lower mass objects ($<30 M_{\mathrm{Jup}}$), likely due to the small number of measured periods for old, low-mass objects. The rotation periods of companion brown dwarfs and planetary-mass objects are consistent with those of isolated objects with similar ages and masses, suggesting similar angular momentum histories. Within the AB Doradus group, we find a high variability occurrence rate and evidence for common angular momentum evolution. The results are encouraging for future variability searches in directly-imaged exoplanets with facilities such as the James Webb Space Telescope and 30-meter telescopes.

==> SED_table.tex <==
\startlongtable
%\begin{longrotatetable}
\begin{deluxetable}{lllllllll}
\tabletypesize{\scriptsize}
\tablecolumns{10}
\tablewidth{0pt}
\setlength{\tabcolsep}{0.05in}
\tablecaption{Fundamental parameters for sample from SED analysis}
%\label{tab:SEDs}
\tablehead{  
\colhead{Shortname} &
\colhead{Parallax$^{a}$ } &
\colhead{Membership} &
\colhead{Age} &
\colhead{$L_{\mathrm{bol}}$} &
\colhead{$T_\mathrm{eff}$} &
\colhead{Radius } & 
\colhead{Mass} &
\colhead{log(g)}\\
\colhead{} &
\colhead{(mas)} &
\colhead{} &
\colhead{(Myr)} &
\colhead{(dex)} &
\colhead{(K)} &
\colhead{($R_{\mathrm{Jup}}$)} & 
\colhead{($M_{\mathrm{Jup}}$)} &
\colhead{(dex)}}

\startdata
\obj{2m0001} & 31.6 $\pm$ 1.8   & HLM ABDMG      & 110--130     & $-3.903\pm0.050$ & $1725\pm5$  & $1.22\pm0.02$      & $32.9\pm3.75$    & $4.73\pm0.06$    \\
\obj{2m0030}  & 41.1$\pm$5.3   & HLM ARG     & 30--50          & $-4.350\pm0.105$ & $1264\pm78$  & $1.36\pm0.04$      & $9.74\pm1.56$    & $4.1\pm0.05$   \\
\obj{2m0031}& 71$\pm$5.0     & HLM CARN      & 150--250         & $-4.353\pm0.062$ & $1343\pm58$  & $1.2\pm0.06$       & $24.42\pm6.93$   & $4.6\pm0.17$     \\
\obj{2m0153} & (19.9$\pm$1.2)  & CAN THA      & 41--49          & $-3.798\pm0.052$ & $1664\pm53$  & $1.48\pm0.03$      & $17.4\pm1.56$    & $4.26\pm0.03$    \\
\obj{2m0326} & (42.7$\pm$2.1)   & HLM ABDMG    & 110--150       & $-4.250\pm0.044$ & $1359\pm46$  & $1.32\pm0.06$      & $18.13\pm4.08$   & $4.37\pm0.11$    \\       
\obj{2m0342}  & (19.4$\pm$1.1)   & HLM THA    & 41--49          &$-3.813\pm0.050$   &$1650\pm51$  &$1.48\pm0.03$       &	$17.25\pm1.52$  & $4.26\pm0.03$   \\
\obj{2m0349} & \nodata    & AM     & 10--150           &\nodata  & \nodata  &\nodata      & \nodata      & \nodata        \\
\obj{2m0355} & 109.6$\pm$0.7   & BF ABDMG      & 110--150       & $-4.116\pm0.006$ & $1527\pm14$  & $1.22\pm0.02$      & $27.82\pm2.09$   & $4.66\pm0.05$     \\
\obj{2m0447} & 23$\pm$3.9     & FLD     & 500--1000              & $-4.278\pm0.148$ & $1521\pm139$ &  $1.02\pm0.07$     & $51.31\pm16.18$   & $5.05\pm0.22$    \\
\obj{2m0459} & (32.2$\pm$3.1)   & HLM ARG     &30--50          & $-4.537\pm0.146$   & $1152\pm98$ & $1.32\pm0.03$      & $8.31\pm1.4$.    & $4.06\pm0.06$   \\
\obj{2m0506} & $59.6\pm5.4$  & FLD     & 500-1000       & $-4.871\pm0.0789$ & $1065\pm63$  & $1.05\pm0.08$       & $26.15\pm7.26$   & $4.74\pm0.2$    \\
\obj{2m0642} & $62.6\pm3.1$  &  CAN ABDMG     & 110--150        & $-4.641\pm0.016$ & $1124\pm11$  & $1.23\pm0.0$       & $11.66\pm0.21$   & $4.28\pm0.01$    \\
\obj{2m0718} & ($107\pm11$)     & CAN BPMG      & 16--28        & $-5.702\pm0.092$ & $596\pm32$   & $1.29\pm0.02$      & $2.56\pm0.35$    & $3.57\pm0.07$    \\
\obj{2m0809} & 42.4$\pm$3.6     & YNG-FLD      & 10--150        & $-4.371\pm0.074$  & $1253\pm74$ & $1.35\pm0.11$      & $12.77\pm7.98$   & $4.12\pm0.36$   \\
\obj{2m0951} & ($17.2\pm1.4$)       & CAN ARG      & 30--50           & $-4.040\pm0.071$ &  $1463\pm65$ & $1.45\pm0.05$      & $ 14.57\pm2.48$  & $4.22\pm0.07$     \\
\obj{2m1551} & 22.1$\pm$1.5     & YNG-FLD       & 10--150       & $-3.864\pm0.059$ & $1653\pm126$ & $1.39\pm0.19$      & $24.12\pm14.07$  & $4.41\pm0.4$    \\
\obj{2m1647} & 42.7$\pm$2.1  & YNG-FLD     & 150--250        & $-4.472\pm0.044$ & $1244\pm47$  & $1.22\pm0.07$      & $18.27\pm6.17$    & $4.45\pm0.19$    \\
\obj{2m1741} & 50.5$\pm$2.9    & BF ABDMG      & 110--150       & $-4.173\pm0.051$ & $1471\pm44$  & $1.23\pm0.02$      & $26.44\pm3.21$   & $4.63\pm0.07$    \\
\obj{2m2002} & 56.7$\pm$1.5     & YNG-FLD       & 10--150       & $-4.299\pm0.024$ & $1301\pm56$  & $1.36\pm0.11$      & $13.22\pm7.89$   & $4.14\pm0.34$    \\
\obj{2m2117}$^{b}$ & 52.4$\pm$ 6.8    & AM/HLM BPMG  & 16--28  & $-4.439\pm0.113$  & $1192\pm80$  & $1.38\pm0.05$      & $7.25\pm1.91$    & $3.95\pm0.12$ \\
             & $76.1\pm3.5$    & AM/FLD    & 500--1000          & $-4.769\pm0.0404$  & $1130\pm50$  & $1.05\pm0.08$      & $27.18\pm7.27$    & $4.75\pm0.21$    \\
\obj{2m2154} & 32.6$\pm$1.0     & CAN CARN       & 150--250     & $-4.138\pm0.028$ & $1539\pm31$  & $1.17\pm0.03$      & $32.7\pm4.18$    & $4.76\pm0.08$    \\
\obj{2m2206+33}& (35.8$\pm$2.4) & CAN ARG      & 30--50         & $-4.669\pm0.059$  & $1076\pm37$  & $1.3\pm0.02$       & $7.59\pm0.9$     & $4.03\pm0.05$    \\
\obj{2m2206-42}  & 33.8$\pm$1.8 & HLM ABDMG    & 110--150       & $-3.945\pm0.045$ & $1684\pm46$  & $1.22\pm0.02$      & $31.86\pm3.45$   & $4.72\pm0.06$     \\
\obj{2m2216}   & (44.2$\pm$3.9) & CAN BPMG       &   16--28     & $-4.949\pm0.077$ & $909\pm41$   & $1.32\pm0.02$      & $4.66\pm1.06$   & $3.79\pm0.12$   \\
\obj{2m2322} & 23.2$\pm$1.0     & BF THA    & 41--49            & $-3.710\pm0.040$ & $1740\pm43$  & $1.5\pm0.03$       & $18.16\pm1.54$   & $4.27\pm0.04$    \\ 
\obj{2m2343} &  (24.7$\pm$1.4)      & CAN ABDMG     & 110-150   &$-3.873\pm0.051$  &  $1755\pm53$ &  $1.22\pm0.02$     &$33.69\pm3.97$     &   $4.74\pm0.06$        \\   \enddata
\label{tab:SEDs}
\tablecomments{The fundamental parameters listed in this table assume membership in the groups listed in the 'Membership' column. Fundamental parameters for candidate and ambiguous members should be treated with caution since their membership is uncertain and may change with updated kinematics.\\  $^{a}$ Parallaxes in parentheses are kinematic distances that assume moving group membership indicated in the membership column. \\ 
$^{b}$ \obj{2m2117} has two discrepant parallax values which result in either high-likelihood $\beta$ Pictoris membership or field membership. We show fundamental parameters for both cases in this table for completeness.}
\end{deluxetable}
%\end{longrotatetable}


==> kinematics.tex <==

\startlongtable
\begin{longrotatetable}
\begin{deluxetable}{lccccccccccc}
\tabletypesize{\scriptsize}
\tablecolumns{10}
\tablewidth{0pt}
\setlength{\tabcolsep}{0.05in}
\tablecaption{Kinematic information for sample.}
%\label{tab:kinematics}
\tablehead{  
\colhead{Name} &
\colhead{$\mu_{\alpha}$ } &
\colhead{$\mu_{\delta}$} &
\colhead{Ref} &
\colhead{RV} &
\colhead{Ref } &
\colhead{Parallax} &
\colhead{Ref } & 
\colhead{LACEwING} &
\colhead{BANYAN $\Sigma$}&
\colhead{Membership}\\
\colhead{} &
\colhead{mas yr$^{-1}$} &
\colhead{mas yr$^{-1}$} &
\colhead{} &
\colhead{km s$^{-1}$} &
\colhead{ } &
\colhead{mas} &
\colhead{} & 
\colhead{} &
\colhead{}&
\colhead{}}

\startdata
%Shortname         & pmra              & pmdec          & Ref     & RV            & Ref             & Parallax  & Ref  \\[0.5ex]  \hline 
\obj*{2m0001} & $143.5\pm4.5$  & $-174.7\pm2.4$  & 1    &  \nodata         & \nodata       & $31.6\pm1.8$   & 1        & 58\% ABDMG     &  92\% ABDMG & HLM\\
\obj*{2m0030}  & $245\pm4$.       & $-28\pm 2$   & 2        &\nodata       &\nodata        & $37.42\pm4.5$  & 11       & 44\% ABDMG     & 87\% ARG  & CAN\\
\obj*{2m0031} & $526\pm 2$       & $-12 \pm4$    & 3         & \nodata     & \nodata       & $71\pm5$       & 12       & 43\% ABDMG      &  98\% CARN & HLM\\
\obj*{2m0153} & $82\pm2.7$       & $-21.3 \pm9.4$& 4       & \nodata       & \nodata       &   \nodata      & \nodata    & 52\% THA        &  89\% THA  & CAN\\
\obj*{2m0326} & $108.0\pm5.0$   & $-156.6\pm4.5$ & 5          &\nodata     & \nodata       &  \nodata       & \nodata   & 56\% ABDMG       & 92\% ABDMG& HLM\\
\obj*{2m0342}  & $73.7\pm2.3$    & $20.6\pm7.8$  & 4         &\nodata      & \nodata       &  \nodata       &  \nodata  &  41\% THA     &  93\% THA   & HLM\\
\obj*{2m0349} & $52.0\pm10.7$   & $-81.9\pm10.3$ & 5  & $13.8\pm3.3$  &    8               &\nodata         &\nodata  & 59\% COL & 55\% BPMG, 20\% ABDMG & CAN\\
\obj*{2m0355} & $219.8\pm1.6$  & $-631.3\pm0.8$  & 1   & $11.92\pm0.22$    & 9             & $109.6\pm0.7$  & 1       & 100\% ABDMG     & 100\% ABDMG & BF\\
\obj*{2m0447} & $20\pm19$     & $-89\pm19$       & 3             & \nodata &\nodata        & $23\pm4$       & 11       &  50\% ABDMG    & 99\% FLD   & AM\\
\obj*{2m0459} & $53.8\pm7.0$   & $84.9\pm7.2$    & 5         & $23.4\pm3.8$& 8             &  \nodata       & \nodata.  & 43\% ARG       &98\% ARG     & HLM\\
\obj*{2m0506} & $46.5\pm9.2$ & $-200.0\pm9.5$    & 5          & \nodata    & \nodata       &  \nodata       &\nodata    & 73\% HYA       & 95\% ABDMG  & HLM\\
\obj*{2m0642} & $3.1\pm 5.3$   & $-397\pm5.3$    & 5           & \nodata   &  \nodata      & $62.6\pm3.1$   & 7        & 69\% ABDMG      &   94\% ABDMG & HLM\\
\obj*{2m0718} & $-175.4\pm13.5$& $254.81\pm13.9$ & 5 & $13\pm2$            & 8             &\nodata         &\nodata     & 90\% ARG        & 85\% BPMG  & CAN\\
\obj*{2m0809} & $-181.9 \pm5.1$    & $-219\pm5.1$& 5     & \nodata         & \nodata       & $42\pm4$       & 11         &  None         & 89\% FLD    &YNG-FLD\\
\obj*{2m0951} & $-92.3\pm9.9$    & $36.8 \pm9.2$ & 5 & $2.8\pm3.3$         & 8             & \nodata        &\nodata     &  35\% ARG      &  87\% ARG &CAN\\
\obj*{2m1551} & $-62.1\pm0.6$ & $-57.7\pm0.6$    & 6   & $-15.2\pm1.1$     & 8             & $22.1\pm1.5$   & 6        &  None      &100\% FLD  & YNG-FLD\\
\obj*{2m1647} & $-178.2\pm4.1$    & $264.2\pm4.7$& 5           & \nodata   & \nodata       & $42.9\pm2.1$   & 12    & 58\% ABDMG   &36\% BPMG, 30\% ARG & CAN \\
\obj*{2m1741} & $-29.2\pm2.1$   & $-356.5\pm 2.1$& 7      & $-0.9\pm3.2$   &  8            & $50.5\pm2.9$   & 7        & 99\% ABDMG     & 99\% ABDMG  &BF\\ 
\obj*{2m2002} &$-111.4\pm3.1$  & $-114.7\pm2.4$  & 1           &  \nodata  & \nodata       & $56.7\pm1.5$   & 1        & None      &100\% FLD  & YNG-FLD\\
\obj*{2m2117} & $148\pm4$      & $-162\pm4$      & 3           & \nodata   &\nodata        & $52.4\pm6.8$   & 12         & 78\% BPMG      & 98\% BPMG & AM$^{\mathrm{a}}$ \\
\obj*{2m2154} & $174.9\pm6.2$    & $-3.3\pm6.1$  & 5     & $-20.7\pm1.0$   & 8             & $32.6\pm1$     & 6        &60\% CARN       & 80\% CARN & CAN\\
\obj*{2m2206+33} & $176\pm9$      & $16\pm11$    & 3          & \nodata    & \nodata       & \nodata        & \nodata    &  24\% ABDMG     & 68\% ARG  &CAN\\
\obj*{2m2206-42} & $130.8\pm1.8$ & $-183.2\pm2.3$& 1         &   \nodata   &\nodata        & $33.8\pm1.8$   & 1        &  79\% ABDMG   &  99\% ABDMG &HLM\\
\obj*{2m2216}   & $160.4\pm14.8$ & $-71.53\pm15.0$& 5         & \nodata    & \nodata       & \nodata        &\nodata     & 33\% ABDMG      & 85\% BPMG &CAN\\
\obj*{2m2322} & $80.1 \pm1.4$  & $-82.0\pm1.6$    & 1        & $6.8\pm0.8$ & 10            & $23.2\pm1.0$   & 1        &  97\% THA    &  99\% THA   &BF\\
\obj*{2m2343} & $124.5\pm5.5$    & $-105.7\pm4.7$ & 5        & \nodata     &  \nodata      &  \nodata       &\nodata     & 37\% THA    &  75\% ABDMG & CAN\\ [0.5ex]  \hline          \enddata
\tablecomments{BF: Bona fide member, HLM: High-likelihood member, CAN: Candidate member, FLD: Field member\\
$^{\mathrm{a}}$ We classify \obj*{2m2117} as ambiguous because \citet{Best2020} and \citet{Kirkpatrick2020} present discrepant parallax values for this target.}
\tablerefs{
(1)~\citet{Gaia2018};
(2)~\citet{Faherty2009}; 
(3)~\citet{Best2015};
(4)~\citet{Gagne2015a};
(5)~\citet{Marocco2021};
(6)~\citet{Liu2016};
(7)~\citet{Kirkpatrick2020};
(8)~Gagn\'e et al. in prep;
(9)~\citet{Blake2010};
(10)~\citet{Faherty2016};
(11)~\citet{Faherty2012};
(12)~\citet{Best2020};
(13)~\citet{Kirkpatrick2011}}
\label{tab:kinematics}
\end{deluxetable}
\end{longrotatetable}



